Sum-of-Squares Lower Bounds for Densest $k$-Subgraph

Given a graph and an integer $k$, Densest $k$-Subgraph is the algorithmic task of finding the subgraph on $k$ vertices with the maximum number of edges. This is a fundamental problem that has been subject to intense study for decades, with applications spanning a wide variety of fields. The state-of-the-art algorithm is an $O(n^{1/4 + \epsilon})$-factor approximation (for any $\epsilon > 0$) due to Bhaskara et al. [STOC '10]. Moreover, the so-called log-density framework predicts that this is optimal, i.e. it is impossible for an efficient algorithm to achieve an $O(n^{1/4 - \epsilon})$-factor approximation. In the average case, Densest $k$-Subgraph is a prototypical noisy inference task which is conjectured to exhibit a statistical-computational gap. In this work, we provide the strongest evidence yet of hardness for Densest $k$-Subgraph by showing matching lower bounds against the powerful Sum-of-Squares (SoS) algorithm, a meta-algorithm based on convex programming that achieves state-of-art algorithmic guarantees for many optimization and inference problems. For $k \leq n^{\frac{1}{2}}$, we obtain a degree $n^{\delta}$ SoS lower bound for the hard regime as predicted by the log-density framework. To show this, we utilize the modern framework for proving SoS lower bounds on average-case problems pioneered by Barak et al. [FOCS '16]. A key issue is that small denser-than-average subgraphs in the input will greatly affect the value of the candidate pseudoexpectation operator around the subgraph. To handle this challenge, we devise a novel matrix factorization scheme based on the positive minimum vertex separator. We then prove an intersection tradeoff lemma to show that the error terms when using this separator are indeed small.

==> basis-comparison.tex <==
\section{Comparison of Fourier and Combinatorial Bases}

For $G \sim \calG_{n,p}$ and a ribbon $R = (A_R, B_R, E(R))$, consider the matrices
\begin{align*}
    M_R^{(Fourier)}[I, J] &= \begin{cases}
    \chi_{E(R)}(G) & I = A_R ,J = B_R\\
    0 & \text{otherwise}
    \end{cases}\\
    M_R^{(combi)}[I, J] &= \begin{cases}
    \left(\frac{1}{p}\right)^{\frac{|E(R)|}{2}} \one_{E(R)}(G) & I = A_R ,J = B_R\\
    0 & \text{otherwise}
    \end{cases}
\end{align*}
The corresponding graph matrices $M_\al^{(Fourier)}, M_\al^{(combi)}$
are formed by summing over all ribbons with the same shape.

The trace of $M_\al^{(combi)}$ (and hence the spectral norm) is fairly nice to express,
\begin{align*}
p^{\frac{|E(R)|}{2}}\tr((M^{(combi)}_\al)^q) &= \sum_{\text{injective } \sigma_1, \dots, \sigma_{q}: V(\al) \to [n]} \prod_{i=1}^q\one_{\sigma_i(V(\al))}(G)\\
&= \sum_{\substack{\text{graphs $H$ formed by identifying}\\ \text{vertices of $V(\al, q)$}}} \left(\text{number of occurrences of $H$}\right)
\end{align*}
Conditioning is already taken care of! If a particular subgraph doesn't appear, then it is zeroed out here.

In the sparse regime with $p$ small, the two matrices are somewhat interchangeable because of the following identity,
\[ \frac{1}{\sqrt{p}}\one_e(G) = \sqrt{p} - \sqrt{1-p}\cdot \chi_e(G)\,.\]
The $\sqrt{p}$ term is the approximation error.

In the dense regime, $\norm{M_\al^{(combi)}} = n^{V(\al) - \frac{|U_\al| + |V_\al|}{2}}$
so it seems like the two matrices are usually not spectrally close.

